Learning Simple Auctions

We present a general framework for proving polynomial sample complexity bounds for the problem of learning from samples the best auction in a class of "simple" auctions. Our framework captures all of the most prominent examples of "simple" auctions, including anonymous and non-anonymous item and bundle pricings, with either a single or multiple buyers. The technique we propose is to break the analysis of auctions into two natural pieces. First, one shows that the set of allocation rules have large amounts of structure; second, fixing an allocation on a sample, one shows that the set of auctions agreeing with this allocation on that sample have revenue functions with low dimensionality. Our results effectively imply that whenever it's possible to compute a near-optimal simple auction with a known prior, it is also possible to compute such an auction with an unknown prior (given a polynomial number of samples).

==> multi-parameter.tex <==
\section{Multi-parameter Auctions}\label{sec:multi-parameter}


In this section, we show that the method of using pseudo-dimension to
measure sample complexity of auctions works more generally than in
single-parameter settings. For several $k$-item multi-parameter
settings where we know a (distribution-dependent) auction earning a
constant factor of the optimal revenue, we show these auctions have
polynomial pseudo-dimension. Thus, one would only need a polynomial
sample of buyers in these settings in order to learn an auction whose
revenue is also a constant of the optimal. The four settings we
consider are, in order of difficulty, a single additive buyer, a set
of $n$ of additive buyers, a set of $n$ unit-demand buyers, and a
single subadditive buyer. In each case, for each buyer, we need that
the valuation of the buyer for each item is ``independent''. The
``simple'' auctions we consider are anonymous and nonanonymous item
and grand bundle pricings. Such auctions are sufficient to earn
revenue which is within a constant factor of the optimal
revenue~\cite{babaioffadditive, chawla2010multi,
  rubensteinsubadditive}.

Grand bundle pricings have constant pseudo-dimension in each of these
cases; the harder work comes from bounding the pseudo-dimension of the
item pricings. Each case reduces to finding a way to apply
Lemma~\ref{lem:param-counting}. The item prices will play the role of
the parameters $x^c_1, \ldots, x^c_d$.  Then, for a fixed set of
samples of size $m$, we partition the item pricings into subclasses.
This partition should have two properties. First, there should not be
too many subclasses (e.g., $\poly(n, m,k)^{\poly(n,k)}$). Second,
fixing a subclass, there should be an encoding of each sample as a
vector such that the revenue of any item pricing (from the class) on
the sample is the dot product between the price vector and the sample
vector. We achieve the second by partitioning the pricings into
classes where the buyer(s) in each sample purchases the same bundle;
each sample's encoding is then a $0/1$ vector describing which items
are purchased within that class.

The difficult part of this in each case is the first step, namely,
showing that there are not too many (e.g., $\exp(m)$ or
$\exp\left(2^{n,k}\right)$) different subclasses.  When a sample is a
single additive buyer, this is straightforward for $m$ fixed
samples. For each item, there are at most $m$ possible selling choices
a pricing has: selling the item to all samples, the $m-1$ with the
higher values for the item, and so on. In total, then, there are at
most $m^k$ assignments of purchased bundles to samples one can achieve
using the $k$ item pricings.

The unit-demand setting, even for a single buyer, doesn't separate
across items this nicely: decreasing the price for item $\k$ might
cause item $\kp$ to stop selling for a fixed sample. However, fixing a
sample, if the the ordering of the differences between each buyers'
item values and item prices is fixed, then so is the
utility-maximizing item, and thus the item purchased (e.g., if
$v_i(\k) - v_{i}(\kp) > \pik{i}{\k} - \pik{i}{\kp}$ for all $\kp\neq \k$,
then $\k$ will be purchased by $i$ on that sample). \footnote{We
  assume ties are broken consistently by the buyer in favor of the
  more expensive item when the utility from buying $\k$ and $\kp$ are
  the same.} So, if the \emph{ordering} between the item price
differences and per-sample item value differences is fixed, for all
buyers in all samples, then the item purchased by each buyer in each
sample will be fixed, and there are at most
$\poly(m,n,k)^{\poly(n,k)}$ of these relative orderings.

Subadditive buyers don't have such a simple statistic which defines
their purchased bundle: in general, a buyer $v$ will buy
$\K = \argmax_{\K} v(\K) - \sum_{\k\in \K} \p(\k)$; trying our trick from
the unit-demand case would require that for all $2^k$ subsets, the
ordering resulting in interleaving the differences in the prices for
each two subsets and the differences in values for each two subsets
for each sample should be fixed, and there might be
${{m\cdot 2^k + 2^k}\choose{2^k}} =
\poly(m, 2^k)^{\exp(k)}$
such orderings. This would only imply an upper bound on the
pseudo-dimension of this class of auctions which is exponential in
$k$, while the class intuitively appears to only have $k$
dimensions. The precise form of the result
of~\citet{rubensteinsubadditive}, however, shows that the better of
grand bundle pricings and a class of auctions even simpler than item
pricings achieves a constant factor of optimal revenue, which doesn't
exhibit this complicated behavior, and we are able to show that this
simpler class does have polynomial pseudo-dimension.

\paragraph{Extensions of notation and definitions}

We will denote a buyer as $i\in[n]$, a sample as $j\in [m]$, a good as
$\k\in[k]$, and a set of goods as $\K\subseteq [k]$. We will denote
$i$th buyer in the $j$th sample's valuation for bundle $\K$ as
$v^j_i(\K)$.  Let $V$ represent some arbitrary set of valuations; we
will instantiate this with different classes when necessary. We say
$V$ is the class of \emph{additive} valuations if, for each $v\in V$
there exist $k$ numbers $v(\kappa)$ such that, for any bundle $\K$,
$v(\K) = \sum_{\k\in\K}v(\kappa)$. Similarly, we will say $V$ is the
set of \emph{unit demand} valuations if for each $v\in V$ there exist
$k$ numbers $v(\kappa)$ such that, for any bundle $\K$,
$v(\K) = \max_{\k\in\K}v(\kappa)$. Finally, we will call $V$ the set
of \emph{subadditive} valuations if, for any $v\in V$, and any bundle
$\K$, for any $\K_1, \K_2$, a bipartition of $\K$, it is the case that
$v(\K) \leq v(\K_1) + v(\K_2)$.

We will consider $4$ types of \emph{pricing} mechanisms, described
now. Any $\p: [k]\to \R_{>0}$ will be called an \emph{anonymous item
  pricing}. We assume any buyer $v$ facing prices $\p$ will buyer her
utility-maximizing bundle
$\K^* = \argmax_{\K\subseteq [k]} v(\K) - \p(\K) = \argmax_\K v(\K) -
\sum_{\k\in \K} \p(\k)$.\footnote{If
  the prices induce indifferences, we assume ties are broken in favor
  of the most expensive bundle.} Then we associate with each $\p$ a
function $f_\p : V \to \R$, representing the revenue of this behavior
for its input valuation:
$f_\p(v) = \p(\K^*) = \sum_{\k\in \K^*} \p(\k)$. Let \itemp denote this
class of functions $f_\p$ for all $\p : [k] \to \R_{\geq 0}$. Similarly,
for any $r\in\R_{> 0}$, we call $r$ an \emph{anonymous grand bundle
  pricing}.  Again, we assume all buyers $v$ facing a grand bundle
price $r$ will buy her utility-maximizing bundle,
$\K^* = \argmax_{\K\in {[k], \emptyset}} v(\K) - r\cdot
\mathbb{I}[\K\neq \emptyset]$.
Let $w_r : V \to \R$ represent the revenue function of such a grand
bundle pricing, $w_r(v) = r\cdot \mathbb{I}[K^*\neq \emptyset]$. We will
refer to the set of $w_r$ (ranging over $r$) as the set \bundlep.

These pricings can be applied to a single buyer. If there are $n$
buyers, for an arbitrary vector $\np \in \left([k] \to \R_{>0}\right)^n$, let
$\fh_{\np} : V^n \to \R$ represent an \emph{individualized item
  pricing} auction with the price for buyer $i$ to buy item $\k$ being
$\pik{i}{\k}$.  We assume there is some fixed, worst-case (for revenue)
order over buyers, and that this order is encoded in the coordinates
of the input to $\fh_\p$ (e.g., $\vec{v}_1$ is the valuation of the
\emph{first} buyer, $\vec{v}_2$ of the second buyer, and so on). Then,
we assume buyer $i$ chooses a utility-maximizing bundle at her prices
of what remains after buyers $1$ through $i-1$ choose their
utility-maximizing bundles. Formally, let
$\K^*_i = \argmax_{\K\subseteq [k]\setminus \cup_{i' <i} \K^*_i} v(\K)
- \sum_{\k\in \K}\pik{i}{\k}$
denote this bundle, and let
$\fh_{\np}(\vec{v}) = \sum_{i\in [n]} \np_i(\K^*_i)$ denote the total
revenue of this individualized pricing applied to buyers
$\vec{v}\in V^n$. Let $\nip$ denote the set of these functions
$\fh_\np$ ranging over all $\np$.  Individualized grand bundle pricings
are defined analogously; let $\ngp$ denote this set of functions.

\subsection{Warm-up: A Single Additive Buyer}\label{sec:additive}
Consider a buyer whose valuation function $v$ has a representation via
$k$ values $v_1, \ldots, v_k$, such that $v(\K) = \sum_{\k\in \K}v_\k$
for any bundle $\K\subseteq [k]$. Then, this buyer is said to have an
additive valuation. Furthermore, suppose the buyer's valuation
$v = (v_1, \ldots, v_k)$ is drawn from a distribution $v \sim \F$. If
there exists some $\F_1, \ldots, \F_k$ such that
$v = (v_1, \ldots, v_k) \sim \F_1 \times \ldots \times \F_k$, we will
say that the distribution over values is independent across items.
Recent work~\cite{babaioffadditive} has shown that either the best
grand bundle pricing or the best item pricing achieves a constant
factor of the optimal revenue when selling to an additive buyer with
independent item valuations. Let $\brev(\F), \prev(\F)$ represent the
revenue of the maximum-revenue bundle pricing and item pricing,
respectively.

\begin{theorem}[Theorem 2, \cite{babaioffadditive}]\label{thm:babaioffadditive}
  Let $\F$ be a joint distribution,
  $\F = \F_1 \times \ldots\times \F_k$. Then, when selling to a single
  additive buyer with valuation $v\sim\F$,
  $6 \cdot \max\{\brev(\F), \prev(\F)\}\geq \rev(\F)$.
\end{theorem}

We now show that these two classes of auctions, for additive bidders,
are simple in a particular sense: namely, they have small
pseudo-dimension.

\begin{theorem}\label{thm:additive-pd}
  Let $\F = \itemp \cup \bundlep$ for a single additive buyer over $k$
  items. Then, the pseudo-dimension of $\F$ is $O(k \log k)$.
\end{theorem}

\begin{proof}
  We prove that a bound on the pseudo-dimension of $\itemp$ and
  $\bundlep$ separately; the pseudo-dimension of $X \cup Y$ is bounded
  by the $2 \max\{\pdim(X),\pdim(Y)\}+1$.

  We begin with bounding the pseudo-dimension of $\bundlep$. Consider
  a set of samples $S$ of size $m$ that can be shattered by $\bundlep$
  with witnesses $(r^1, \ldots, r^m)$. As in the single-dimensional
  case, we will partition the auctions into equivalence classes whose
  number of labelings of $S$ we will count separately. We will call
  $\w_\rho, \w_{\rho'}\in\bundlep$ equivalent if, after sorting
  $v^j([k]) = \sum_{\k\in [k]} v^j(\{\k\})$, inserting $\rho$ and
  $\rho'$ into this sorting (while maintaining the list's sortedness)
  partitions these values into the same two sets for $\rho$ and
  $\rho'$. Let $\C_\ell$ be some equivalence class formed by this
  definition. Then, let $g^{\C_\ell}(v^j) = 1$ if $v^j$ buys the grand
  bundle according to $\C_\ell$ (which is fixed in $\C_\ell$). Let
  $x^\rho = \rho$; thus,
  $g^{\C_\ell}(v^j) \cdot x^\rho = \w_\rho(v^j)$.
  Lemma~\ref{lem:param-counting} then implies \bundlep can induce at
  most $(2m+1) \cdot m^{3}$ labelings of $S$; since $S$ is
  shatterable, this implies $2^m \leq (2m+1) \cdot m^{3}$, so
  $m \leq 3$ and $\pdim(\bundlep) \leq 3$.

  We now bound the pseudo-dimension of $\itemp$. Consider a set of
  samples $S$ of size $m$ that can be shattered by $\itemp$ with
  witnesses $(r^1, \ldots, r^m)$.  We will call $f_{\p}, f_{\p'}$
  equivalent if, after sorting the values $v^j({\k})$ for each $j$ and
  $\k$, and sorting the numbers $\p(\k), \p'(\k)$, merging the two
  sortings has the same ordering between the values (e.g., $\p(\k)$ is
  in the same location in the sorted list as is $\p'(\k)$, for all
  $\k$). Notice then that two item pricings are equivalent if and only
  if they would sell the same sets of items to each sample, and there
  are at most ${mk + k}\choose{k}$ such equivalence classes.  Then,
  one can define $g^{\C_\ell}(v^j)\in \{0,1\}^{k}$ for a given
  equivalence class $\C_{\ell}$ such that $g^{\C_\ell}(v^j)_\k= 1$ if
  and only if sample $v^j$ purchases item $\k$ for auctions in
  $\C_\ell$.  Define $x^\p_\k = \p(\k)$ for all $\p$. Then, for any
  $\p\in \C_\ell$, $x^p\cdot g^{\C_\ell}(v^j) = f_\p(v^j)$, so
  applying Lemma~\ref{lem:param-counting}, we have that $\C$ induces
  at most $ (mk + k)^{k} \cdot m^{k+2}$ labelings. Thus, since $S$ is
  shatterable,

\[2^m \leq (m(k+1))^{2k  + 2}\]
implying $m = O( k\log k)$, so $\pdim(\itemp) = O( k\log k)$, and thus

\[\pdim(\itemp \cup \bundlep) = O(k\log k)\] thus completing the proof. \end{proof}

Thus, combining Theorems~\ref{thm:additive-pd}
and~\ref{thm:babaioffadditive}, we have the following corollary
describing the sample complexity of learning approximately optimal
auctions for additive buyers.

\begin{corollary}\label{cor:additive-sample}
  Suppose $\F = \F_1 \times \ldots \times \F_k$ is a product
  distribution over $[0,H]^k$. Then, with probability $1-\delta$, the
  empirical revenue maximizer $f \in \itemp\cup\bundlep$ over $m$
  samples drawn from $\F$ has expected revenue at least
  $\frac{1}{6} - \eps$ times the optimal expected revenue when selling
  to additive buyers $v\sim \F$, if

\[m \geq \left(\frac{H}{\eps}\right)^2\left(k\log k \ln\left(\frac{H}{\epsilon}\right) + \ln\left(\frac{1}{\delta}\right)\right).\]
\end{corollary}

\subsection{Moving to Multiple Additive Buyers}\label{sec:multiple-additive}

This section shows how one can bound the number of samples needed to
learn an approximately optimal auction when selling to \emph{multiple}
additive buyers. This work requires the recent reduction
of~\citet{yao2015}, which shows one can separate the problem of
optimally selling to $n$ additive buyers into solving $n$ optimal
selling problems for one buyer, one for each buyer. Informally, his
work shows that it suffices to consider only ever selling an item to
the \emph{highest bidder for that item}. Then, one can separately
optimize the way in which these items are sold to the highest bidder
for them; either one can solve this problem optimally or
approximately; in either case, one gets an approximation to the
optimal, unseparated problem.

More formally, fix some vector $\beta\in \R^k$.  We call a
single-buyer mechanism $\A_i$ $\beta$-restricted if, for any $v_i$ and
for all $\k\in[k]$, $\A_i(v_i)$ sells item $\k$ to $v_i$ only if
$v_i(\k) > \beta_\k$. Suppose some mechanism $\bA_i$ takes \emph{as
  input} a vector $\beta^i$ along with $v_i$, and chooses an
allocation and payment for $i$ subject to being
$\beta^i$-restricted. We will call such a mechanism a parametrically
restricted mechanism.  Fix some input $v$, and let
$\beta^i_\k = \max_{i'\neq i} v_{i'}(\k)$.  For a fixed (parametric)
restricted mechanism $\bA_i$ for each $i$, let
$(\bA_1, \ldots, \bA_n)$ represent the mechanism which allocates to
buyer $i$ according to $\bA_i$ for each $i$, using as input for the
restriction $\beta^i$.

Let \sp denote the second-price mechanism (which sells each item
separately to the highest bidder at the second-highest bidder's bid).
Finally, let
$\maxmech_\F(\A, \B) = \argmax_{y\in \{\A, \B\}} \E_{v\sim
  \F}[\rev(y(v))]$
denote the higher revenue mechanism of $\A, \B$ in expectation over
the draw of a sample. The following theorem of~\citet{yao2015} shows
that, when buyers' valuations are drawn independently for each item,
one can ``separate'' the problem of revenue maximization into $n$
single-buyer optimizations.

\begin{theorem}\label{thm:yaomultiple}[Corollary of Theorem 2~\citep{yao2015}]
  Suppose $\vec{v} \sim \F = \F_1 \times \ldots \times \F_k$ and
  $\F_\k \in [0, \infty]^n$.   Suppose
  $\bA_{i}$ is an $\alpha$-approximately revenue optimal parametrically restricted mechanism for
  selling to buyer $i$ according to $\F$. Then,
  $(\bA_{1}, \ldots, \bA_{n})$ is a feasible
  mechanism, and
  \[\maxmech_\F((\bA_{1}, \ldots \bA_{n}), \sp)\]
  achieves a $\frac{1}{8\alpha+1}$-fraction of the optimal revenue for
  $\F$.
\end{theorem}

We now show that combining this result with
Theorem~\ref{thm:babaioffadditive} of~\citet{babaioffadditive} gives
us a class of mechanisms for selling to $n$ additive buyers which has
polynomial (in $n$ and $k$) pseudo-dimension which always contains
a constant-factor approximation to the optimal mechanism.  This class
will contain individualized item and individualized bundle pricings,
subject to these pricings only selling item $\k$ to bidder $i$ if $i$
is the strictly highest bider for $\k$. 

Intuitively, one of these classes should contain a pricing which
achieves high welfare, according to
Theorem~\ref{thm:babaioffadditive}. However, this theorem only describes the
near-optimality of pricings in the unrestricted case. We show that
restricted pricings are also approximately optimal with respect to all
restricted mechanisms.  We do this by transforming both the pricings
and bids, and show an equivalence. We transform buyer $i$'s bid
$(v_i(1), \ldots, v_i(k))$ into a bid $(\bv_i(1), \ldots, \bv_i(k))$
where $\bv_i(\k) = v_i(\k)\cdot \I\lbrack v_i(\k) > \beta^i_\k\rbrack$
is only above $0$ if buyer $i$ bid strictly more than $\beta^i_\k$ on
item $\k$.

We will refer to individualized item pricings as
$\np : ([k] \to \R_{>0})^n$, and an item pricing for player $i$ as
$\np_i : [k] \to \R_{>0}$.  With respect to a single bidder's item pricing
$\np_i$, we will use $\bpi{i} : \R^k_{> 0}\to \left([k] \to \R_{>0}\right)$ to represent
a \emph{modified} pricing, such that
$\bpi{i}(\beta^i)_\k = \max (\beta^i_\k, \pik{i}{\k})$ for all $\k$ and
all $\beta^i$.  For an individualized pricing $\np$, let
%
\[\nf_{\np}(v) = \sum_{i}f_{\bpi{i}(\beta^i)}(\bv_i),\]
%
the revenue of running the $\beta^i$-restricted version of $\np_i$ on
$\bv$ for each $i$ separately.  Then, we represent the class of these
functions as

\[\bitemp = \{\nf_{\np} : V^n  \to \R | \np\in\R^{n\times k}_{>0}, \nf_\np(v) =\sum_i f_{\bpi{i}(\beta^i)}(\bv_i)\}.\]

Similarly, for an individualized grand bundle pricing
$\nr\in\R^n_{>0}$, let $\nri{i} \in\R$ represent bidder $i$'s grand
bundle price. Let $\br{i}$ denote the 
the modified grand bundle pricing for bidder $i$ such that
$\bri{i}(\beta^i) = \max (\sum_{\k : \bv_i(\k) > 0} \beta^i_\k, \nri{i})$ for the
bundle of items such that $\bv_i(\k) > 0$. Then, fixing an individualized  bundle
pricing $\nr$, let
%
\[\nw_{\nr}(v) = \sum_{i}w_{\bri{i}(\beta^i)}(\bv_i),\]
%
the revenue of running the $\beta^i$-restricted version of $\nr_i$ on
$\bv$ for each $i$ separately. The class of these functions will be
represented as
%
\[\bbundlep = \{\nw_{\nr} :  V^n  \to \R | \nr\in\R^n_{>0}, \nw_\nr(v) = \w_{\bri{i}(\beta^i)}(\bv_i)\}.\]

In order to show that this class of modified mechanisms (which are
parametrically restricted and IC/IR, by Lemma~\ref{lem:restricted})
for the modified bid for buyer $i$ still contain an approximately
optimal restricted mechanism for the original buyer $i$, we need to
show several things. First, it must be that
$(\bv_i(1), \ldots, \bv_i(k))$ is still drawn from some product
distribution (Lemma~\ref{lem:independent}). Next, we need to show
that, fixing a modified bid $\bv$, the $\beta^i$-restriction increases
the revenue pointwise for each fixed item pricing
(Lemma~\ref{lem:item-increase}) and each fixed grand bundle pricing
(Lemma~\ref{lem:bundle-increase}). Then, these things together will
imply that running the best (parametrically restricted) item or grand
bundle pricing for buyer $i$ on the modified valuation $\bv_i$ will
achieve a constant fraction of the optimal revenue possible when
selling to $v_i$ using any $\beta^i$-restricted mechanism. Thus, these
mechanisms will be approximately optimal for selling to $\v$, even
when comparing to the best unrestricted
mechanism (Theorem~\ref{thm:equiv-reduced}).


The following theorem states formally that these classes contain a
constant-factor approximation to the revenue-optimal auction for
$\F$.

\begin{theorem}\label{thm:equiv-reduced}
  The set $\itemp\cup\bundlep$ contain a $6$-approximation to the
  revenue-optimal mechanism for selling to $\bv_i$.  Let $\A_i$ be the
  mechanism which maximizes the expected revenue from this class for
  buyer $i$. Then, 
\[\maxmech_\F((\bA_{1}, \ldots \bA_{n}), \sp)\]
  achieves a $\frac{1}{49}$-fraction of the optimal revenue for
  $\v \sim \F_1 \times \ldots \times \F_k$.
\end{theorem}

The proof of Theorem~\ref{thm:equiv-reduced} follows the statement of
several lemmas we will use in its proof.  The following lemma states
that the modified item and grand bundle pricings are, in fact,
parametrically restricted (and incentive compatible and individually
rational).

\begin{lemma}\label{lem:restricted}
  Consider any fixed item pricing $\npi{i}$ or grand-bundle pricing
  $\nri{i}$. For any $v$, both $\bpi{i}(\beta^i)$ and $\bri{i}(\beta^i)$ (defined with respect to
  $\beta^i_\k = \max_{i'\neq i}v_{i'}(\k)$) when run on $\bv_i$ are
  $\beta^i$-restricted, and are incentive-compatible and individually
  rational.
\end{lemma}

The next lemma shows that modifying $v_i$ to $\bv_i$ maintains the
independence of the item values of buyer $i$.

\begin{lemma}\label{lem:independent}
  Suppose $v\sim \F^1\times \ldots \times \F^k$. Then, for any $i$, there exists
  $\F'^1, \ldots \F'^k$ such that $\bv_i \sim \F'^1 \times \ldots \times \F'^k$. 
\end{lemma}

The following two lemmas state that running the restricted item or
bundle pricings on the modified valuations only improves the revenue
of each pointwise.

\begin{lemma}\label{lem:item-increase}
  Fix any $\v$, and the corresponding $\beta^i$. For any
  $\npi{i} \in \R^k_{>0}$ and corresponding $\bpi{i}$,
  \[\rev(\npi{i}, \bv_i) \leq \rev(\bpi{i}(\beta^i), \bv_i).\]
\end{lemma}
\begin{lemma}\label{lem:bundle-increase}
Fix any $\v$ and the corresponding $\beta^i$. For any $\nri{i} \in \R_{> 0}$ and corresponding $\bri{i}$, 
  \[\rev(\nri{i}, \bv_i) \leq \rev(\bri{i}(\beta^i), \bv_i).\]
\end{lemma}

We now present the proof of Theorem~\ref{thm:equiv-reduced}, the main
``representation'' proof of this section.

 \begin{prevproof}{Theorem}{thm:equiv-reduced}
   First, the set of (unmodified) item pricings and grand bundle
   pricings contain a $6$-approximation to the revenue-optimal
   mechanism for selling to $\bv_i$, since $\bv_i$ is independent
   across items (Lemma~\ref{lem:independent}), by
   Theorem~\ref{thm:babaioffadditive}. Then, by
   Lemmas~\ref{lem:item-increase} and~\ref{lem:bundle-increase}, the
   set of modified item pricings and grand bundle pricings only have
   pointwise higher revenue than their unmodified counterparts when
   selling to $\bv_i$, so these classes also contain a
   $6$-approximation. Let $\bA_{i} = \bpi{i}$ if $\bpi{i}$ was the
   revenue-optimal restricted pricing, or $\bA_{i} = \bri{i}$ if
   $\bri{i}$ was the revenue-optimal restricted pricing.  Thus,
   $\bA_{i}$ is a $6$-approximation to the revenue-maximizing
   $\beta^i$-restricted auction for buyer $\bv_i$. Furthermore, it is
   $\beta^i$-restricted (Lemma~\ref{lem:restricted}).

   Finally, we claim that any optimal $\beta^i$-restricted
   incentive-compatible mechanism achieves the same revenue selling to
   $v_i$ as to $\bv_i$. This follows from the fact that any allocation
   which is $\beta^i$-restricted can be sold to both $v_i$ and
   $\bv_i$, and $v_i$ and $\bv_i$ would be willing to pay the same
   price for any allocation which is $\beta^i$-restricted (since no
   item $\k$ for which $v_i(\k) \leq \beta^i_\k$ is in any such
   allocation). Thus, the revenue for this optimal mechanism will be
   the same in both cases or it could be strictly improved by offering
   the higher-revenue menu to both $v_i$ and $\bv_i$ (and all
   valuations in between).

   Thus, the optimal $\beta^i$-restricted mechanism for $v_i$ achieves
   the same revenue on $\bv_i$. Thus, since $\bA_{i}$ is a
   $6$-approximation to the revenue-optimal auction on $\bv_i$, it is
   also a $6$-approximation to the revenue-optimal
   $\beta^i$-restricted auction on $v_i$. Thus, by
   Theorem~\ref{thm:yaomultiple}, the claim follows.
\end{prevproof}



The following theorem states that these two classes have polynomial
pseudo-dimension, which will imply learnability over the class with a
polynomial sample (Corollary~\ref{cor:samples-multi-add}).

\begin{theorem}\label{thm:pseudo-multi-add}
  Let $\bitemp, \bbundlep$ denote the set of parametrically restricted item
  and bundle pricings. Then,
  \[\pdim\left(\bitemp \cup\bbundlep\cup\{\sp\}\right) = O\left(n\cdot k \ln\left(n\cdot k\right)\right).\]
\end{theorem}


\begin{proof}
  Notice that second-price is a single auction, so has VC dimension 1. 

  We will argue that both $\bitemp$ and $\bbundlep$ separately satisfy
  this bound.  Fix a sample $S = (v^1, \ldots, v^m)$, of $m$ valuation
  profiles (and for each $j\in [m]$, $v^j_i$ represents the valuation
  of buyer $i$ in sample $j$). We will upper-bound $m$ for any $S$
  which is shatterable. For a fixed sample, the relative ordering of
  $v^j_i(\k)$ and $v^{j'}_{i'}(\k')$ for all
  $i,i' \in [n], \k, \k'\in[k], j, j'\in[m]$ is fixed; thus, the
  highest and second-highest bidder for each item $\k$ on each sample
  $j$ are fixed (and thus, the only possible winner of item $\k$ on
  $j$ is fixed). Let $\win{j}{\k}, \second{j}{\k}$ represent the
  highest and second-highest bidder for $\k$ on sample $j$ (breaking
  ties consistently across samples and items).

  For each of $\bitemp, \bbundlep$ separately, we will partition the
  set of selling procedures into sets $C_1, \ldots, C_\alpha$, such
  that within a given $C_t$, \emph{each} bidder, from \emph{each}
  sample, purchases the same items and pays the same linear
  combination of parameters of selling parameters and other bidders'
  bids.

  We begin with restricted item pricings.  For some restricted pricing
  $\bnp$, let $x^{\bnp}$ denote a $(n+1)\cdot k$ dimensional vector,
  where $x^{\bnp}_{i, \k} = \pik{i}{\k}$ denotes the $i$th bidder's
  (unrestricted) price for item $\k$, and $x^{\bnp}_{n+1, \k} = 1$ for
  all $\k$.  We will call two restricted item pricings $\bnp, \bnp'$
  \emph{equivalent} if, letting $\np, \np'$ denote their unrestricted
  pricing counterparts,
\begin{itemize}
\item The relative order of $\pik{i}{\k}$ and $\pik{i'}{\k'}$ is the same as for $\ppik{i}{\k}$ and
  $\ppik{i'}{\k'}$ for all $\k, \k'\in [k]$, $i,i'\in[n]$.
\item The interleaving of the sorted values $\pik{i}{\k}$ with the
  $m\cdot n \cdot k$ values $v^j_{i'}(\k')$ for all
  $j\in [m], i, i'\in[n], \k, \k' \in [k]$ induces the same partition
  as does the interleaving of the sorted values $\ppik{i}{\k}$.
\end{itemize}

Then, define each $C_\ell$ to be an equivalence class defined by this
equivalence relation.  Note that
\[\alpha = (nk)! \cdot {{m\cdot n \cdot k + n\cdot k}\choose {n\cdot k}} =
O\left(\left((m +1)\cdot n \cdot k\right)^{2n\cdot k}\right).\]
Fix some $C_\ell$.  We will show there exists an
$(n + 1) \cdot k$-dimensional vector $g^{C_\ell}(v^j)$ such that, for
every $\bnp\in C_\ell$,
$g^{C_\ell}(v^j) \cdot x^{\bnp} = \nf_{\np}(v^j)$ (the revenue of
running the restricted individualized item pricings on $v^j$). Notice
that, fixing $C_\ell$, on each $v^j$, each highest bidder's payment
for $\k$ is fixed to be either $0$ (if there is a tie for the highest
bid $\k$ on $j$, or the highest bidder's price is higher than her
bid), the second highest bid for $\k$ on $v^j$ (when the second
highest bid for $\k$ is more than the winner's unrestricted price for
$\k$), or the winner's unrestricted price for $\k$, since the latter
two numbers have a fixed relative order.
Thus, we can define
\[
 g^{C_\ell}(v^j)_{i,\k} =
  \begin{cases} 
      \hfill 1    \hfill & \text{$i = \win{j}{\k}$ and is paying her unrestricted price for $\k$}\\
      \hfill 0 \hfill & \text{$i = \win{j}{\k}$ but either $i$ pays second price for $\k$, or $v^j_{i}(\k) < \pik{i}{\k}$}\\
      \hfill 0  \hfill & \text{$i \in [n]$ but either $i \neq \win{j}{\k}$ or there is a tie $v^j_{\win{j}{\k}}(\k) = v^j_{\second{j}{\k}}(\k)$}\\
      \hfill v^j_{\second{j}{\k}}(\k) & i  = n+1 \text{ and $\win{j}{\k}$ is paying  second price for $\k$}\\
  \end{cases}.
\]
 Then, for any $\bnp\in C_\ell$, we have that
 \[x^{\bnp} \cdot g^{C_\ell}(v^j) = \sum_{\k : \win{j}{\k}\textrm{ pays
     second price for $\k$ on $j$ }} v^j_{\second{j}{\k}} + \sum_{\k :
   \win{j}{\k}\textrm{ pays unrestricted price for $\k$ on $j$ }}
 \pik{\win{j}{\k}}{ \k} = \nf_\bp(v^j)\]
 as desired. Then, Lemma~\ref{lem:param-counting} implies there are at
 most
 $\alpha \cdot m^{(n+1)\cdot k} = {(m+1)\cdot n\cdot k \choose n\cdot
   k} \cdot m^{(n+1)\cdot k}$,
 implying $m = O\left(n\cdot k \ln\left(n\cdot k\right)\right)$ if
 the set is shatterable.

 A similar argument holds for restricted bundle pricings, with the
 equivalence class defined slightly differently.  For a restricted
 bundle pricing $\bnr$, define $x^{\bnr}$ to be the
 $n+1$-dimensional vector, where $x^{\bnr}_{i} = \nr_i$ for
 $i\in [n]$ and $x^{\bnr}_{i} = 1$ for $i = n+1$.  Two restricted
 bundle pricings $\bnr, \bnr'$ are said to be equivalent if, for
 their unrestricted versions $\nr, \nr'$,
\begin{itemize}
\item The relative order of $\nr_{i}, \nr_{i'}$ is the same as  $\nr'_{i}, \nr'_{i'}$ for all $i,i'$.
\item For each sample $j$ and each bidder $i$, that the relative order
  of $\nr_i$, $\pay{i}{j} = \sum_{\k : \win{j}{\k} = i, v^j_i(\k) > v^j_{\second{j}{\k}}(\k)}
  v^j_{\second{j}{\k}}(\k)$ and  $ \bidk{i}{j} = \sum_{\k : \win{j}{k} = i, v^j_i(\k) > v^j_{\second{j}{\k}}(\k)}
  v^j_{i}(\k)$ is the same as for $\nr'_i, \pay{i}{j}$, and $\bidk{i}{j}$.
\end{itemize}
Notice that $\bidk{i}{j}$ denotes the sum of the (strictly) winning
bids that bidder $i$ makes on sample $j$, or the \emph{value} bidder
$i$ gets from winning this bundle. Similarly, $\pay{i}{j}$ denotes the
sum of the second-highest bids for those items, or the \emph{price}
for this bundle for $i$, if $i$ pays second-price.  Again, these two
rules imply that equivalent bundle pricings have the same form of
payments on all samples, for all buyers. That is, fixing some
$C_\ell$, on each samples $j$, each bidder $i$ either loses all items,
pays her unrestricted bundle price for her winning items, or pays
second price for the items she wins.  Let $C_1, \ldots, C_\alpha$ be
the equivalence classes defined by this rule. There are at most
$\alpha = n! \cdot {mn +n\choose n }$ classes. For each class
$C_\ell$, let
\[
 g^{C_\ell}(v^j)_{i} =
  \begin{cases} 
    \hfill 1    \hfill & \text{$i$ wins some items and pays her unrestricted bundle price}\\
    \hfill 0  \hfill & \bidk{i}{j} \text{ is strictly less than $i$'s unrestricted bundle price}\\
    \hfill 0  \hfill & \text{$i \neq \win{j}{\k}$ for all $\k$}\\
    \hfill 0 \hfill & \text{$i$ pays second price for her bundle}\\
    \hfill \sum_{\k : \textrm{ $\win{j}{k}$ pays second price }}v^j_{\second{j}{\k}}(\k) & i  = n+1 \text{ (The sum of the second prices any bidders pay)}\\
  \end{cases}.
\]
As before, $x^{\bnr} \cdot g^{C_\ell}(v^j) = \ng{}(v^j)$, so
Lemma~\ref{lem:param-counting} implies that the set of restricted
bundle pricings induce at most $\alpha \cdot m^{n+3}$ labelings,
implying $m \leq O\left(n \ln(n)\right)$ if the set is shatterable, as desired.
\end{proof}

\begin{corollary}\label{cor:samples-multi-add}
  It is possible to learn a $\frac{1}{49} - \eps$-approximately
  optimal auction for selling to $n$ additive bidders, if bidder's
  valuations $v_i\sim \F_i = \F^1_i\times \ldots \times \F^k_i$ are
  independent across items, with sample complexity
\[ m = O\left(\left(\frac{Hn}{\epsilon}\right)^2 n\cdot k \ln(n\cdot k)\log\frac{Hn}{\epsilon} + \log\frac{1}{\delta}\right).\]
\end{corollary}
\subsection{Unit-demand buyers}\label{sec:unit-demand}

In this section, we show how to extend our methods from the previous
sections to a setting where buyers' valuations have substitutes: when
buyers are unit-demand. We assume there are $n$ buyers whose
valuations $v_i : 2^k \to \R$ are unit-demand: $i$'s value can be
described by $k$ numbers $v_i(1), \ldots, v_i(k)$ such that
$v_i(\K) = \max_{\k\in \K} v_i(\k)$ for every $K$. In this case, we
will abuse notation and allow $v_i \in \R^k$ to be a $k$-dimensional
vector representing these $k$ values.  If
$v_i \sim \F_i = \F^1_i \times \ldots \times \F^k_i$, we will say that $v$ is
independent across items.  Again, our starting point is a
result~\cite{chawla2010multi} showing that, when
$v_i\sim F_i^1\times\ldots\times F_i^k$ is drawn independently across
items for each unit-demand bidder, independetly for each buyer, the
best item pricing achieves at least $\frac{1}{10.67}$ of the optimal
expected revenue. We recall that our definition of individualized item
pricings assume that bidder $1$ first chooses her most-preferred
bundle according to $\np_1$, bidder $2$ then selects her
most-preferred bundle from those items remaining at $\p_2$, and so on.
\begin{theorem}[\citet{chawla2010multi}]\label{thm:chawlaud}
  If $v_i\sim \F_i^1 \times \ldots \times \F_i^k$ represents a unit-demand bidder $i$'s 
  $k$-dimensional valuation, then there exists some $\np\in\nip$ such that
  $\rev_\F(\np) \geq \frac{1}{10.67}\rev(\F)$.
\end{theorem}

We now show how to bound the pseudo-dimension of item pricings for a
collection of $n$ unit-demand buyers. The proof is analagous to the
additive case, but with a twist: whether or not buyer $i$ buys $\k$
depends on \emph{all} her prices, not just $\pik{i}{\k}$. On the other
hand, there are a small number of quantities (namely, for all
$j, i, \k, \k'$, the set of differences $v^j_i(\k) - v^j_{i}(\k')$ and
$\pik{i}{\k}- \pik{i}{\kp}$) whose relative ordering completely
determines the purchased bundle.

\begin{theorem}\label{thm:unit-pd}
  For $n$  unit-demand buyers, in a setting with $k$ items,
  \[\pdim( \nip) = O\left((nk)^2 \log \left(nk\right)\right).\]
\end{theorem}

\begin{proof}
  Let $S$ be a set of size $m$ which is shatterable by $\nip$ with
  witnesses $(r^1, \ldots, r^m)$. We will again separate the auctions
  into equivalence classes. We call two auctions $f_{\np}, f_{\np'}$
  equivalent if merging the sorted list of the $m(nk)^2$ quantities
  $v^j_i(\k) - v^j_{i}(\k')$ (for each $j, i, k, k'$) and the sorted
  list of the $(nk)^2$ quantities $\pik{i}{\k} - \pik{i}{\k'}$ (for
  each $i, \k,\k'$) results in the same ordering as does merging the
  former list with the sorted list of $\ppik{i}{\k} - \ppik{i}{\k'}$s.
  There are then at most ${mk^2 + k^2}\choose {k^2}$ such equivalence
  classes of auctions. Furthermore, within a given auction class
  $\C_\ell$, for each sample $j$, for each buyer $i$, there is one
  item $\k$ such that
  $v^j_{i}(\k) - v^j_{i}(\k') \geq \pik{i}{\k} - \pik{i}{\k'}$ for all
  $\np$ such that $f_{\np} \in \C_\ell$. Thus, for each sample, within
  an auction class $\C_{\ell}$, each buyer within that sample will
  purchase the same item. Let $g^{C_\ell}(v^j)_{i,\k} = 1$ if, on
  sample $j$, $i$ buys $\k$ for the pricings in $\C_\ell$.  Let
  $x^{\np}_{i,\k} = \pik{i}{\k}$. Thus,
  $g^{C_\ell}(v^j) \cdot x^\np = f_\np(v^j)$.
  Lemma~\ref{lem:param-counting} then implies there are at most
  ${{mn^2k^2 + n^2k^2}\choose {n^2k^2}} \cdot m^{nk+2}$ labelings of
  these $m$ points using $\C$. If $S$ is shatterable, for
  $k\geq 2$,

\[2^m \leq (mn^2k^2 + n^2k^2)^{n^2k^2}\cdot m^{nk+2} \leq (2mn^2k^2)^{2nk^2}\]
or $m \leq 8n^2k^2 \log(nk)$, which implies the desired bound.
\end{proof}

Theorem~\ref{thm:unit-pd} immediately implies the following sample
complexity bound for such unit-demand settings.

\begin{corollary}\label{cor:unit-sample}
  Suppose $v_i \sim \F_i = \F_i^1 \times \ldots \times \F_i^k$ is a
  product distribution over $[0,H]^k$ for all $i\in[n]$. Then, with
  probability $1-\delta$, the empirical revenue maximizer $f \in \nip$
  over $m$ samples drawn from $\F$ has expected revenue at least
  $\frac{1}{10.67} - \eps$ times the optimal expected revenue when selling
  to unit-demand buyers $v\sim \F$, if

\[m \geq \left(\frac{H}{\eps}\right)^2\left(k^2n^2\log k \ln\left(\frac{H}{\epsilon}\right) + \ln\left(\frac{1}{\delta}\right)\right).\]
\end{corollary}

\subsection{Learning auctions for a subadditive
  buyer}\label{sec:subadditive}

The previous section highlighted one difficulty in proving bounds on
the pseudo-dimension in settings with substitutes: the problem doesn't
separate across items. In the case of unit-demand items, it is
sufficient to consider the ordering of the pairwise differences
between items' values and their prices to determine which items will
be purchased by each buyer for each sample; fixing this ordering, the
items purchased by each item per sample will be fixed. For a single
subadditive buyer facing item prices, the bundle purchased can depend
much more delicately on the set of $k$ prices. As mentioned
previously, partitioning the auctions into sets where the difference
between each pair of bundles' pricings and values are fixed would
induce $\Omega\left(\left(m\cdot 2^{k^2}\right)^{2^{k^2}} \right)$
distinct sets. Lemma~\ref{lem:param-counting} would then imply at best
a bound on pseudodimension exponential in $k$.

However, the result of~\citet{rubensteinsubadditive} actually shows
one need not have a subadditive buyer implementing a demand oracle
(which might purchase arbitrary bundles given appropriate prices)
against item prices to get a constant approximation to revenue.
Instead, the guarantee holds even if a buyer facing item pricings $\p$
only purchased an item $\k$ if $\k$ is the unique item for which
$v^j(\k)\geq \p(\k)$. One can then replace a standard item pricing
auction with its pointwise revenue-reduced item pricing, which only
get revenue from the sampled buyers for which exactly one item's value
is larger than its price. \footnote{One would need not run the
  revenue-reduced item pricing to get the guaranteed revenue, only to
  estimate empirical revenue on the training set; selecting the item
  pricing based on its revenue-reduced empirical revenue would imply
  the revenue the true item pricing would achieve would be at least as
  good.} Furthermore, any two revenue-reduced item pricings which
agree on the ordering of the per-item values of a sample and the
per-item prices will sell the same item to that sample, and receive
revenue equal to that item's price. There are at most $\poly(m,k)^{k}$
of these relative orderings, since one is only interleaving per-item
prices rather than prices for bundles; this yields the desired
polynomial pseudodimension bound fora subadditive bidder facing
reduced item pricings.

For the remainder of this section, we will need some slightly
different notation. For any $\p\in \R^k$, let
%
\[h_{\p}(v^j) = \sum_{\k\in[k]}\p(\k)\cdot \mathbb{I}[\k\textrm{ is the unique item
  for which }v^j(\k) \geq \p(\k)],\]
%
and let $\ritemp = \{ h_{\p} | \p\in \R^k\}$. We will identify
$f_{\p}\in \itemp$ with $h_{\p}\in \ritemp$ to be the standard item
pricing for a given revenue-reduced item pricing.  Let $\rprev(\F)$
denote the revenue achievable by the best revenue-reduced item pricing
on $\F$. We now state an observation suggested by these names: namely,
that any revenue-reduced item pricing has pointwise worse revenue than
its non-revenue-reduced item pricing counterpart.
\begin{observation}\label{obs:reduced}
For any $\p$,  for $f_{\p}\in \itemp, h_{\p}\in \ritemp$,
\[f_{\p} (v) \geq h_{\p}(v),\]
for any $v\in \R^k$; thus, $\prev(\F) \geq \rprev(\F)$.
\end{observation}

In order to state the main result of~\citet{rubensteinsubadditive}
(and this section of our paper), we must define what notion of
independence across items is sufficient to achieve constant revenue
approximations using item and grand bundle pricings.
\begin{definition}[\citet{rubensteinsubadditive}]
  A distribution $\F$ over valuation functions $v : 2^k \to \R$ is
  subadditive over independent items if:
\begin{enumerate}
\item  All $v$ in the support of $\F$ are monotone; $v(\K\cup\K') \geq v(\K)$ for all $\K,\K'$.
\item  All $v$ in the support of $\F$ are subadditive: $v(\K \cup \K') \leq v(\K) + v(\K')$ for all $\K, \K'$.
\item All $v$ in the support of $\F$ exhibit no externalities: there
  exists some $\F^{\vec x}$ over $\R^k$ and a function $V$ such that
  $\F$ is a distribution that samples $\vec x \sim \F^{\vec x}$ and
  outputs $v$ such that $v(\K) = V(\{x_\k\}_{\k\in \K}, \K)$ for all $\K$.
\item $\F^{\vec x}$ is product across its $k$ dimensions.
\end{enumerate}
\end{definition}

Now, we state the main result of~\citet{rubensteinsubadditive}, which
we use as a building block for our main theorem of the section.

\begin{theorem}[\citet{rubensteinsubadditive}]\label{thm:rubenstein}
  Let $\F$ be a distribution over subadditive buyers which is independent across items. Then, there is
  a universal constant $c$ (independent of $\F$) such that, for $v\sim\F$,
\[\max\{\brev_\F(v), \rprev_\F(v)\} \geq c \cdot \rev_\F(v).\]
\end{theorem}

We now state our main structural result of the section, which bounds
the pseudo-dimension of $\rprev$ and $\brev$ in the setting with a
subadditive buyer.

\begin{theorem}\label{thm:subadditive-pd}
  For a single subadditive buyer in a setting with $k$ items,
  \[\pdim(\ritemp \cup \bundlep) = O\left(k\log k\right).\]
\end{theorem}
\begin{proof}
  The proof that $\pdim(\bundlep) \leq 3$ is identical to the additive
  case; it remains to show that
  $\pdim(\ritemp) = O\left(k \log k\right)$. Fix a sample $S$ of size
  $m$ with witnesses $r^1, \ldots, r^m$ which can be shattered.
  Consider $h_{\p}, h_{\p'}$ equivalent if, after sorting the values
  $v^j(\k)$ for all $j$ and $\k$, and sorting $\p(\k)$ (and $\p'(\k)$),
  merging these sorted lists yields the same ordered list. Then, for
  an equivalent class of auctions $C_{\ell}$, any sample $j$ has a
  fixed sale: their is either one item $\k^j$ which this class of
  auctions $C$ sells to sample $j$, or all of $C_{\ell}$ sells sample
  $j$ no item. There are at most ${mk + k}\choose{k}$ such
  interleavings (and thus, equivalence classes).

  Then, fixing the equivalence class of auctions $C_{\ell}$, encode
  sample $j$ as a $k$-dimensional vector $g^{C_\ell}(v^j)$.  If there
  is some $\k^j$ for $v^j$ in $C_\ell$, set
  $g^{C_\ell}(v^j_{\k^j}) = 1$ and $g^{C_\ell}(v^j_\k) = 0$ for all
  other $\k$.  Encode each auction $h_\p$ as $x^\p_\k = \p(\k)$ for
  $\k\in[k]$. Then, $h_\p(v^j) = g^{C_\ell}(v^j) \cdot x^\p$ for
  $\p\in C_\ell$. 

  Thus, Lemma~\ref{lem:param-counting} implies that there are at most
  ${mk + k}\choose{k} \cdot m^{k+2}$ labelings of $S$ using these
  auctions.Thus, since $S$ is shatterable,
  \[2^m \leq {{mk+ k}\choose{k}} \cdot m^{k+2} \leq (2km)^{3k}\]
  implying $m = O(k\log k)$.
\end{proof}

\begin{corollary}\label{cor:subadditive-sample}
  Let $f$ be the empirical revenue maximizer of
  $\ritemp \cup \bundlep$ on $m$ samples from $\F$ which is
  subadditive and independent across $k$ items. Then, with probability
  $1-\delta$, $\rev(\hat{f}, \F) \geq (c - \epsilon)\cdot \rev(\F)$,
  where
\[\hat{f} =  \begin{cases} 
      \w & \w\in\bundlep \\
      f_{\p} & g = h_{\p}\in\ritemp
   \end{cases}
\]
so long as 
\[m \geq \left(\frac{H}{\eps}\right)^2\left(k\log k \ln\left(\frac{H}{\epsilon}\right) + \ln\left(\frac{1}{\delta}\right)\right).\]
\end{corollary}




==> prelims.tex <==

\section{Preliminaries}\label{sec:prelim}

This section reviews useful terminology and notation standard in
Bayesian auction design and learning theory.

\paragraph{Bayesian Auction Design}\label{sec:bayesian}

We consider \emph{single-parameter settings} with $n$ bidders.
This means that each bidder has a single unknown parameter, its {\em
  valuation} or willingness to pay for ``winning.''
(Every bidder has value~0 for losing.)
A setting is specified by a
collection $\mathcal{X}$ of subsets of $\{1,2,\ldots,n\}$; each such
subset represent a collection of bidders that can simultaneously
``win.''  For example, in a setting with $k$ copies of an item, where
no bidder wants more than one copy, $\mathcal{X}$ would be all subsets
of $\{1,2,\ldots,n\}$ of cardinality at most~$k$.

A generalization of this case, studied in Section~\ref{sec:matroid},
is {\em matroid} settings.  These satisfy: (i) whenever $X \in \X$ and
$Y \subseteq X$, $Y \in \X$; and (ii) for two sets $|I_1| < |I_2|$,
$I_1, I_2 \in \X$, there is always an augmenting element
$i_2 \in I_2 \setminus I_1$ such that $I_1 \cup \{i_2\}\in \X$, $\X$.
Section~\ref{sec:single-param} also considers arbitrary
single-parameter settings, where the only assumption is that
$\emptyset \in \X$.  To ease comprehension, we often illustrate our
main ideas using single-item auctions (where $\X$ is the singletons
and the empty set).

We assume bidders' valuations are drawn from the continuous joint
cumulative distribution $\F$.  Except in the extension in
Section~\ref{sec:mhr}, we assume that the support of $\F$ is limited to
$[1,H]^n$.  As in most of optimal auction
theory~\cite{myerson1981optimal}, we usually assume that $\F$ is a
product distribution, with $\F= \F_1\times \F_2 \times \ldots \times \F_n$
and each $v_i \sim \F_i$ drawn independently but not identically.
%; we will
%mention explicitly where independence is needed for some results. 
The \emph{virtual value} of bidder $i$ is denoted by
$\phi_i(v_i) = v_i - \frac{1-\F_i(v_i)}{\f_i(v_i)}$.  A distribution
satisfies the \emph{monotone-hazard rate (MHR)} condition if
$\f_i(v_i)/(1-\F_i(v_i))$ is nondecreasing; intuitively, if its tails
are no heavier than those of an exponential distribution.  In a
fundamental paper, \cite{myerson1981optimal} proved that when every
virtual valuation function is nondecreasing (the ``regular'' case),
the auction that maximizes expected revenue for $n$ Bayesian bidders
chooses winners in a way which maximizes the sum of the virtual values
of the winners. This auction is known as Myerson's auction, which we
refer to as $\M$. The result can be extended to the general,
``non-regular'' case by replacing the virtual valuation functions by
``ironed virtual valuation functions.''  The details are
well-understood but technical; see~\citet{myerson1981optimal} and
%When $ \phi_i$ is not weakly increasing (i.e., $F_i$ is
%not {\em regular}), the optimal auction \emph{ironed} virtual value $\bar\phi_i(v_i)$,
%which is monotone, can be used instead (for details,
\citet{hartline2015} for details.
%). For settings where agents are not assumed
%to be regular, running $\M$ with respect to the ironed virtual
%valuation functions maximizes the expected revenue over all
%incentive-compatible mechanisms.



\paragraph{ Sample Complexity, VC Dimension, and the
  Pseudo-Dimension}\label{sec:learning}

This section reviews several well-known definitions from learning
theory. Suppose there is some domain $\dom$, and let $c$ be some
unknown target function $c: \dom \to \{0,1\}$.  Let $\F$ be an unknown
distribution over $\dom$. We wish to understand how many labeled
samples $(x, c(x))$, $x\sim \F$, are necessary and sufficient to be
able to output a $\hat c$ which agrees with $c$ almost everywhere with
respect to $\F$. The distribution-independent sample complexity of
learning $c$ depends fundamentally on the ``complexity'' of the set of
binary functions $\C$ from which we are choosing $\hat c$.  We define
the relevant complexity measure next.

Let $S$ be a set of $m$ samples from $\dom$. The set $S$ is said to be
\emph {shattered} by $\C$ if, for every subset $T\subseteq S$, there is
some $c_T\in\C$ such that $c_T(x) = 1$ if $x\in T$ and $c_T(y) = 0$ if
$y\notin T$.  That is, ranging over all $c \in \C$ induces all
$2^{|S|}$ possible projections onto $S$.
The {\em VC dimension} of $\C$, denoted $\VC(\C)$, is the size
of the largest set $S$ that can be shattered by $\C$. 

Let $\err_S(\hat c) = (\sum_{x\in S} |c(x) - \hat{c}(x)|)/|S|$ denote
the empirical error of $\hat c$ on $S$, and let
$\err(\hat c) = \E_{x\sim D}[|c(x) - \hat{c}(x)|]$ denote the
true expected error of $\hat c$ with respect to $\F$.  A key
result from learning theory~\cite{VC} is: for every distribution $\F$,
a sample $S$ of size
$\Omega (\eps^{-2}(\VC(\C) + \ln\frac{1}{\delta}))$ is sufficient to
guarantee that
$\err_{S}(\hat c) \in [\err(\hat c) - \epsilon, \err(\hat c) +
\epsilon]$
for \emph{every} $\hat c\in \C$ with probability $1-\delta$.  In this
case, the error on the sample is close to the true error,
simultaneously for every hypothesis in $\C$.  In particular, choosing
the hypothesis with the minimum sample error minimizes the true error,
up to $2\eps$. We say $\C$ is {\em $(\epsilon, \delta)$-uniformly
  learnable with sample complexity $m$} if, given a sample $S$ of size
$m$, with probability $1-\delta$, for all $c\in \C$,
$|\err_S(c) - \err(c)| < \epsilon$: thus, any class $\C$ is
$(\eps, \delta)$-uniformly learnable with
$m = \Theta\left(\frac{1}{\eps^2}\left(\VC(\C) + \ln
    \frac{1}{\delta}\right)\right)$
samples.  Conversely, for every learning algorithm $\A$ that uses
fewer than $\frac{\VC(\C)}{\epsilon}$ samples, there exists a
distribution $\F'$ and a constant $q$ such that, with probability at
least $q$, $\A$ outputs a hypothesis $\hat c'\in \C$ with
$\err(\hat c') > \err(\hat c) + \frac{\epsilon}{2}$ for some
$\hat c \in \C$.  That is, the true error of the output hypothesis is
more than $\frac{\epsilon}{2}$ larger the best hypothesis in the
class.

To learn real-valued functions, we need a generalization of VC
dimension (which concerns binary functions). The
\emph{pseudo-dimension} \cite{pollard1984} does exactly
this.\footnote{The {\em fat-shattering dimension} is a weaker
  condition that is also sufficient for sample complexity bounds.  All
  of our arguments give the same upper bounds on the pseudo-dimension
  and the fat-shattering dimension of various auction classes, so we
  present the stronger statements.} Formally, let $c : \dom \to [0,H]$
be a real-valued function over $\dom$, and $\C$ the class we are
learning over. Let $S$ be a sample drawn from $\F$, $|S|=m$, labeled
according to $c$.  Both the empirical and true error of a hypothesis
$\hat c$ are defined as before, though $|\hat c(x) - c(x)|$ can now
take on values in $[0, H]$ rather than in $\{0,1\}$. Let
$(r^1, \ldots, r^m) \in [0,H]^m$ be a set of \emph{targets} for
$S$. We say $(r^1, \ldots, r^m) $ \emph{witnesses} the shattering of
$S$ by $\C$ if, for each $T\subseteq S$, there exists some $c_T\in \C$
such that $f_T(x^i) \geq r^i$ for all $x^i \in T$ and $c_T(x^i) < r^i$
for all $x^i \notin T$. If there exists some $\vec r$ witnessing the
shattering of $S$, we say $S$ is {\em shatterable} by $\C$.  The {\em
  pseudo-dimension} of $\C$, denoted $\pd_\C$, is the size of the
largest set $S$ which is shatterable by $\C$.  The sample complexity
upper bounds of this paper are derived from the following theorem,
which states that the distribution-independent sample complexity of
learning over a class of real-valued functions $\C$ is governed by the
class's pseudo-dimension.

\begin{theorem}\label{thm:fat-sample}[E.g.~\cite{AB}]
  Suppose $\C$ is a class of real-valued functions with range in $[0,H]$ and
  pseudo-dimension $\pd_\C$. For every $\epsilon > 0, \delta \in [0,1]$, the
  sample complexity of $(\epsilon, \delta)$-uniformly learning $f$
  with respect to $\C$ is $ m = O\left(
    \left(\frac{H}{\epsilon}\right)^2\left(\pd_\C\ln\left(\frac{H}{\epsilon}\right)
      + \ln\left(\frac{1}{\delta}\right)\right)\right).$
\end{theorem}
Moreover, the guarantee in Theorem~\ref{thm:fat-sample}
is realized by the learning algorithm that simply outputs the
function $c \in \C$ with the smallest empirical error on the sample.

\paragraph{Applying Pseudo-Dimension to Auction
  Classes}\label{sec:applying}


For the remainder of this paper, we consider classes of truthful
auctions $\C$.\footnote{An auction is {\em truthful} if truthful
  bidding is a dominant strategy for every bidder.  That is: for every
  bidder~$i$, and all possible bids by the other bidders, $i$
  maximizes its expected utility (value minus price paid) by bidding
  its true value.  In the single-parameter settings that we study,
the expected revenue of the optimal non-truthful auction (measured at
a Bayes-Nash equilibrium with respect to the prior distribution) is no
larger than that of the optimal truthful auction.}
When we discuss some auction $c\in \C$, we treat
$c : [0,H]^n \to \mathbb{R}$ as the function that maps (truthful) bid
tuples to the revenue achieved on them by the auction $c$.  Then,
rather than minimizing error, we aim to maximize revenue.  In our
setting, the guarantee of Theorem~\ref{thm:fat-sample} directly
implies that, with probability at least $1-\delta$ (over the $m$
samples), the output of the {\em empirical revenue maximization}
learning algorithm --- which returns the auction $c \in \C$ with the
highest average revenue on the samples --- chooses an auction with
expected revenue (over the true underlying distribution $\F$) that is
within an additive $\eps$ of the maximum possible. 




==> rw-new.tex <==

\subsection{Related Work}\label{sec:related}

The present work shares much of its spirit and
high-level goals with~\citet{balcan2008reducing}, who
%Ten years ago, the prescient paper of~\citet{balcan2008reducing}
%(following~\citet{B+03} and~\citet{blum2005near}) showed that
%statistical learning theory provides a framework for answering all of
%these questions, and 
proposed applying 
%the framework 
statistical learning theory to the design of
near-optimal auctions.  
%The present work revisits this idea under a
%stronger assumption --- replacing the prior-free assumption used
%in~\citet{balcan2008reducing} with a distributional model --- which
%gives results in much more general auction environments and tighter
%connections to both learning theory and Bayesian-optimal auction
%theory.
The first-order
difference between the two works is that our work assumes bidders'
valuations are drawn from an unknown distribution, while
~\citet{balcan2008reducing} study the more demanding ``prior-free''
setting. Since no auction can achieve near-optimal revenue
ex-post,
%~\cite{G+06},~
\citet{balcan2008reducing} define their revenue
benchmark with respect to a set $\G$ of auctions on each input $\vals$
as the maximum revenue obtained by any auction of $\G$ on $\vals$.
The idea of learning from samples enters the work
of~\citet{balcan2008reducing} through the internal randomness of their
partitioning of bidders, rather than through an exogenous distribution
over inputs (as in this work). Both our work and theirs requires
polynomial dependence on $H, \tfrac{1}{\eps}$: ours in terms of a
necessary number of samples, and theirs in terms of a necessary number
of bidders; as well as a measure of the complexity of the class $\G$
(in our case, the pseudo-dimension, and in theirs, an analagous
measure).  The primary improvement of our work over of the results
in~\citet{balcan2008reducing} is that our results apply for single
item-auctions, matroid feasibility, and arbitrary single-parameter
settings (see Section~\ref{sec:prelim} for definitions); while their
results apply only to single-parameter settings 
of unlimited 
supply.\footnote{See~\citet{balcan2007CMUtechreport} for an extension
to the case of a large finite supply.} We also view as a feature the
fact that our sample complexity upper bounds can be deduced directly
from well-known results in learning theory --- we can focus instead on
the non-trivial and problem-specific work of bounding the
pseudo-dimension and representation error of well-chosen auction
classes.


\citet{elkind2007} also considers a similar model to ours, but only
for the special case of single-item auctions.  While her proposed
auction format is similar to ours, our results cover the far more
general case of arbitrary single-parameter settings and and non-finite
support distributions; our sample complexity bounds are also better
even in the case of a single-item auction (linear rather than
quadratic dependence on the number of bidders).  On the other hand,
the learning algorithm in \cite{elkind2007} (for single-item auctions)
is computationally efficient, while ours is not.

\citet{CR14} study single-item auctions with $n$ bidders with
valuations drawn from independent (not necessarily identical)
``regular'' distributions (see Section~\ref{sec:prelim}), and prove
upper and lower bounds (polynomial in $n$ and $\eps^{-1}$) on the
sample complexity of learning a $(1-\eps)$-approximate auction.  While
the formalism in their work is inspired by learning theory, no formal
connections are offered; in particular, both their upper and lower
bounds were proved from scratch. Our positive results include
single-item auctions as a very special case and, for bounded or MHR
valuations, our sample complexity upper bounds are much better than
those in~\citet{CR14}.

\citet{huang2014making} consider learning the optimal price from
samples when there is a single buyer and a single seller; this problem
was also studied implicitly in~\cite{dhangwatnotai2010revenue}.  Our
general positive results obviously cover the bounded-valuation and MHR
settings in \cite{huang2014making}, though the specialized analysis in
\cite{huang2014making} yields better (indeed, almost optimal) sample
complexity bounds, as a function of $\eps^{-1}$ and/or $H$.

\citet{medina2014learning} show how to use a combination of the
pseudo-dimension and Rademacher complexity to measure the sample
complexity of selecting a single reserve price for the  VCG mechanism
to optimize revenue.  In our notation, this corresponds to analyzing a
single set~$\C$ of auctions (VCG with a reserve).
\citet{medina2014learning} do not address the expressivity
vs.\ simplicity trade-off that is central to this paper.

\citet{dughmi2014sampling} also study the sample complexity of learning good
auctions, but their main results are negative (exponential sample
complexity), for the difficult scenario of multi-parameter settings.
(All settings in this paper are single-parameter.)

Our work on $t$-level auctions also contributes to the literature on
simple approximately revenue-maximizing auctions (e.g.,
\cite{chawla2007algorithmic,hartline2009simple,
  chawla2010multi,devanur2011prior,
  RTY12,yao2015soda,moshematt2014focs}).  Here, one takes the
perspective of a seller who knows the valuation distribution $\F$ but
is bound by a ``simplicity constraint'' on the auction deployed,
thereby ruling out the optimal auction.  Our results that bound the
representation error of $t$-level auctions
(Theorems~\ref{thm:rep-bounded},~\ref{thm:rep-mhr},~\ref{thm:rep-matroid},
and~\ref{thm:rep-param}) can be interpreted as a principled way to
trade off the simplicity of an auction with its approximation
guarantee.  While previous work in this literature generally left the
term ``simple'' safely undefined, this paper effectively proposes the
pseudo-dimension of an auction class as a rigorous and quantifiable
simplicity measure.

Finally, our results for in multi-parameter settings rely on the
constant-factor revenue approximation guarantees for item and
grand-bundle pricing when a single buyer is
additive~\cite{babaioffadditive} or
subadditive~\cite{rubensteinsubadditive}, and, in the mutiple
unit-demand setting, that per-person item pricings achieve a constant
factor of optimal revenue~\cite{chawla2010multi}. Moreover, by
the recent result of~\citet{yao2015}, the better of (individualized)
grand bundle and item pricings earn a constant factor of the optimal
revenue for $n$ additive buyers; we can also bound the
pseudo-dimension of this class of auctions. Grand bundle pricings,
anonymous item pricings, and individualized item pricings have only
$1, k$, and $nk$ parameters, respectively.  This might suggest a
simple proof of polynomial pseudodimension; however, the complexity of
these auctions arises from the complicated behavior of a non-additive
buyer facing item prices, which may depend delicately on arbitrary
subsets of the prices.



==> yaoreduction.tex <==

Consider a buyer whose valuation function $v$ has a representation via
$k$ values $v_1, \ldots, v_k$, such that $v(\K) = \sum_{\k\in \K}v_\k$
for any bundle $\K\subseteq [k]$. Then, this buyer is said to have an
additive valuation. Furthermore, suppose the buyer's valuation
$v = (v_1, \ldots, v_k)$ is drawn from a distribution $v \sim \F$. If
there exists some $\F_1, \ldots, \F_k$ such that
$v = (v_1, \ldots, v_k) \sim \F_1 \times \ldots \times \F_k$, we will
say that the distribution over values is independent across items.
Recent work~\cite{babaioffadditive} has shown that either the best
grand bundle pricing or the best item pricing achieves a constant
factor of the optimal revenue when selling to an additive buyer with
independent item valuations. Let $\brev(\F), \prev(\F)$ represent the
revenue of the maximum-revenue bundle pricing and item pricing,
respectively.

\begin{theorem}[Theorem 2, \cite{babaioffadditive}]\label{thm:babaioffadditive}
  Let $\F$ be a joint distribution,
  $\F = \F_1 \times \ldots\times \F_k$. Then, when selling to a single
  additive buyer with valuation $v\sim\F$,
  $6 \cdot \max\{\brev(\F), \prev(\F)\}\geq \rev(\F)$.
\end{theorem}


\subsection{Moving to Multiple Additive Buyers}\label{sec:multiple-additive}

This section shows how one can bound the number of samples needed to
learn an approximately optimal auction when selling to \emph{multiple}
additive buyers. This work requires the recent reduction
of~\citet{yao2015}, which shows one can separate the problem of
optimally selling to $n$ additive buyers into solving $n$ optimal
selling problems for one buyer, one for each buyer. Informally, his
work shows that it suffices to consider only ever selling an item to
the \emph{highest bidder for that item}. Then, one can separately
optimize the way in which these items are sold to the highest bidder
for them; either one can solve this problem optimally or
approximately; in either case, one gets an approximation to the
optimal, unseparated problem.

More formally, fix some vector $\beta\in \R^k$.  We call a
single-buyer mechanism $\A_i$ $\beta$-restricted if, for any $v_i$ and
for all $\k\in[k]$, $\A_i(v_i)$ sells item $\k$ to $v_i$ only if
$v_i(\k) > \beta_\k$. Suppose some mechanism $\bA_i$ takes \emph{as
  input} a vector $\beta^i$ along with $v_i$, and chooses an
allocation and payment for $i$ subject to being
$\beta^i$-restricted. We will call such a mechanism a parametrically
restricted mechanism.  Fix some input $v$, and let
$\beta^i_\k = \max_{i'\neq i} v_{i'}(\k)$.  For a fixed (parametric)
restricted mechanism $\bA_i$ for each $i$, let
$(\bA_1, \ldots, \bA_n)$ represent the mechanism which allocates to
buyer $i$ according to $\bA_i$ for each $i$, using as input for the
restriction $\beta^i$.

Let \sp denote the second-price mechanism (which sells each item
separately to the highest bidder at the second-highest bidder's bid).
Finally, let
$\maxmech_\F(\A, \B) = \argmax_{y\in \{\A, \B\}} \E_{v\sim
  \F}[\rev(y(v))]$
denote the higher revenue mechanism of $\A, \B$ in expectation over
the draw of a sample. The following theorem of~\citet{yao2015} shows
that, when buyers' valuations are drawn independently for each item,
one can ``separate'' the problem of revenue maximization into $n$
single-buyer optimizations.

\begin{theorem}\label{thm:yaomultiple}[Corollary of Theorem 2~\citep{yao2015}]
  Suppose $\vec{v} \sim \F = \F_1 \times \ldots \times \F_k$ and
  $\F_\k \in [0, \infty]^n$.   Suppose
  $\bA_{i}$ is an $\alpha$-approximately revenue optimal parametrically restricted mechanism for
  selling to buyer $i$ according to $\F$. Then,
  $(\bA_{1}, \ldots, \bA_{n})$ is a feasible
  mechanism, and
  \[\maxmech_\F((\bA_{1}, \ldots \bA_{n}), \sp)\]
  achieves a $\frac{1}{8\alpha+1}$-fraction of the optimal revenue for
  $\F$.
\end{theorem}

We now show that combining this result with
Theorem~\ref{thm:babaioffadditive} of~\citet{babaioffadditive} gives
us a class of mechanisms for selling to $n$ additive buyers which has
polynomial (in $n$ and $k$) pseudo-dimension which always contains
a constant-factor approximation to the optimal mechanism.  This class
will contain individualized item and individualized bundle pricings,
subject to these pricings only selling item $\k$ to bidder $i$ if $i$
is the strictly highest bider for $\k$. 

Intuitively, one of these classes should contain a pricing which
achieves high welfare, according to
Theorem~\ref{thm:babaioffadditive}. However, this theorem only describes the
near-optimality of pricings in the unrestricted case. We show that
restricted pricings are also approximately optimal with respect to all
restricted mechanisms.  We do this by transforming both the pricings
and bids, and show an equivalence. We transform buyer $i$'s bid
$(v_i(1), \ldots, v_i(k))$ into a bid $(\bv_i(1), \ldots, \bv_i(k))$
where $\bv_i(\k) = v_i(\k)\cdot \I\lbrack v_i(\k) > \beta^i_\k\rbrack$
is only above $0$ if buyer $i$ bid strictly more than $\beta^i_\k$ on
item $\k$.

We will refer to individualized item pricings as
$\np : ([k] \to \R_{>0})^n$, and an item pricing for player $i$ as
$\np_i : [k] \to \R_{>0}$.  With respect to a single bidder's item pricing
$\np_i$, we will use $\bpi{i} : \R^k_{> 0}\to \left([k] \to \R_{>0}\right)$ to represent
a \emph{modified} pricing, such that
$\bpi{i}(\beta^i)_\k = \max (\beta^i_\k, \pik{i}{\k})$ for all $\k$ and
all $\beta^i$.  For an individualized pricing $\np$, let
%
\[\nf_{\np}(v) = \sum_{i}f_{\bpi{i}(\beta^i)}(\bv_i),\]
%
the revenue of running the $\beta^i$-restricted version of $\np_i$ on
$\bv$ for each $i$ separately.  Then, we represent the class of these
functions as

\[\bitemp = \{\nf_{\np} : V^n  \to \R | \np\in\R^{n\times k}_{>0}, \nf_\np(v) =\sum_i f_{\bpi{i}(\beta^i)}(\bv_i)\}.\]

Similarly, for an individualized grand bundle pricing
$\nr\in\R^n_{>0}$, let $\nri{i} \in\R$ represent bidder $i$'s grand
bundle price. Let $\br{i}$ denote the 
the modified grand bundle pricing for bidder $i$ such that
$\bri{i}(\beta^i) = \max (\sum_{\k : \bv_i(\k) > 0} \beta^i_\k, \nri{i})$ for the
bundle of items such that $\bv_i(\k) > 0$. Then, fixing an individualized  bundle
pricing $\nr$, let
%
\[\nw_{\nr}(v) = \sum_{i}w_{\bri{i}(\beta^i)}(\bv_i),\]
%
the revenue of running the $\beta^i$-restricted version of $\nr_i$ on
$\bv$ for each $i$ separately. The class of these functions will be
represented as
%
\[\bbundlep = \{\nw_{\nr} :  V^n  \to \R | \nr\in\R^n_{>0}, \nw_\nr(v) = \w_{\bri{i}(\beta^i)}(\bv_i)\}.\]

In order to show that this class of modified mechanisms (which are
parametrically restricted and IC/IR, by Lemma~\ref{lem:restricted})
for the modified bid for buyer $i$ still contain an approximately
optimal restricted mechanism for the original buyer $i$, we need to
show several things. First, it must be that
$(\bv_i(1), \ldots, \bv_i(k))$ is still drawn from some product
distribution (Lemma~\ref{lem:independent}). Next, we need to show
that, fixing a modified bid $\bv$, the $\beta^i$-restriction increases
the revenue pointwise for each fixed item pricing
(Lemma~\ref{lem:item-increase}) and each fixed grand bundle pricing
(Lemma~\ref{lem:bundle-increase}). Then, these things together will
imply that running the best (parametrically restricted) item or grand
bundle pricing for buyer $i$ on the modified valuation $\bv_i$ will
achieve a constant fraction of the optimal revenue possible when
selling to $v_i$ using any $\beta^i$-restricted mechanism. Thus, these
mechanisms will be approximately optimal for selling to $\v$, even
when comparing to the best unrestricted
mechanism (Theorem~\ref{thm:equiv-reduced}).


The following theorem states formally that these classes contain a
constant-factor approximation to the revenue-optimal auction for
$\F$.

\begin{theorem}\label{thm:equiv-reduced}
  The set $\itemp\cup\bundlep$ contain a $6$-approximation to the
  revenue-optimal mechanism for selling to $\bv_i$.  Let $\A_i$ be the
  mechanism which maximizes the expected revenue from this class for
  buyer $i$. Then, 
\[\maxmech_\F((\bA_{1}, \ldots \bA_{n}), \sp)\]
  achieves a $\frac{1}{49}$-fraction of the optimal revenue for
  $\v \sim \F_1 \times \ldots \times \F_k$.
\end{theorem}

The proof of Theorem~\ref{thm:equiv-reduced} follows the statement of
several lemmas we will use in its proof.  The following lemma states
that the modified item and grand bundle pricings are, in fact,
parametrically restricted (and incentive compatible and individually
rational).

\begin{lemma}\label{lem:restricted}
  Consider any fixed item pricing $\npi{i}$ or grand-bundle pricing
  $\nri{i}$. For any $v$, both $\bpi{i}(\beta^i)$ and $\bri{i}(\beta^i)$ (defined with respect to
  $\beta^i_\k = \max_{i'\neq i}v_{i'}(\k)$) when run on $\bv_i$ are
  $\beta^i$-restricted, and are incentive-compatible and individually
  rational.
\end{lemma}

The next lemma shows that modifying $v_i$ to $\bv_i$ maintains the
independence of the item values of buyer $i$.

\begin{lemma}\label{lem:independent}
  Suppose $v\sim \F^1\times \ldots \times \F^k$. Then, for any $i$, there exists
  $\F'^1, \ldots \F'^k$ such that $\bv_i \sim \F'^1 \times \ldots \times \F'^k$. 
\end{lemma}

The following two lemmas state that running the restricted item or
bundle pricings on the modified valuations only improves the revenue
of each pointwise.

\begin{lemma}\label{lem:item-increase}
  Fix any $\v$, and the corresponding $\beta^i$. For any
  $\npi{i} \in \R^k_{>0}$ and corresponding $\bpi{i}$,
  \[\rev(\npi{i}, \bv_i) \leq \rev(\bpi{i}(\beta^i), \bv_i).\]
\end{lemma}
\begin{lemma}\label{lem:bundle-increase}
Fix any $\v$ and the corresponding $\beta^i$. For any $\nri{i} \in \R_{> 0}$ and corresponding $\bri{i}$, 
  \[\rev(\nri{i}, \bv_i) \leq \rev(\bri{i}(\beta^i), \bv_i).\]
\end{lemma}

We now present the proof of Theorem~\ref{thm:equiv-reduced}, the main
``representation'' proof of this section.

 \begin{prevproof}{Theorem}{thm:equiv-reduced}
   First, the set of (unmodified) item pricings and grand bundle
   pricings contain a $6$-approximation to the revenue-optimal
   mechanism for selling to $\bv_i$, since $\bv_i$ is independent
   across items (Lemma~\ref{lem:independent}), by
   Theorem~\ref{thm:babaioffadditive}. Then, by
   Lemmas~\ref{lem:item-increase} and~\ref{lem:bundle-increase}, the
   set of modified item pricings and grand bundle pricings only have
   pointwise higher revenue than their unmodified counterparts when
   selling to $\bv_i$, so these classes also contain a
   $6$-approximation. Let $\bA_{i} = \bpi{i}$ if $\bpi{i}$ was the
   revenue-optimal restricted pricing, or $\bA_{i} = \bri{i}$ if
   $\bri{i}$ was the revenue-optimal restricted pricing.  Thus,
   $\bA_{i}$ is a $6$-approximation to the revenue-maximizing
   $\beta^i$-restricted auction for buyer $\bv_i$. Furthermore, it is
   $\beta^i$-restricted (Lemma~\ref{lem:restricted}).

   Finally, we claim that any optimal $\beta^i$-restricted
   incentive-compatible mechanism achieves the same revenue selling to
   $v_i$ as to $\bv_i$. This follows from the fact that any allocation
   which is $\beta^i$-restricted can be sold to both $v_i$ and
   $\bv_i$, and $v_i$ and $\bv_i$ would be willing to pay the same
   price for any allocation which is $\beta^i$-restricted (since no
   item $\k$ for which $v_i(\k) \leq \beta^i_\k$ is in any such
   allocation). Thus, the revenue for this optimal mechanism will be
   the same in both cases or it could be strictly improved by offering
   the higher-revenue menu to both $v_i$ and $\bv_i$ (and all
   valuations in between).

   Thus, the optimal $\beta^i$-restricted mechanism for $v_i$ achieves
   the same revenue on $\bv_i$. Thus, since $\bA_{i}$ is a
   $6$-approximation to the revenue-optimal auction on $\bv_i$, it is
   also a $6$-approximation to the revenue-optimal
   $\beta^i$-restricted auction on $v_i$. Thus, by
   Theorem~\ref{thm:yaomultiple}, the claim follows.
\end{prevproof}


\subsection{Multiple Additive Buyers}
\begin{prevproof}{Lemma}{lem:restricted}
  We first show these mechanisms are $\beta^i$-restricted. Since
  $\bv_i(\k) > 0$ only if $\v_i(\k) > \beta^i_\k$ neither $\bpi{i}(\beta^i)$ nor
  $\bpi{i}(\beta^i)$ will sell item $\k$ to $\bv_i$ unless $v_i(\k) > \beta^i_\k$,
  thus both are $\beta^i_\k$-restricted.

  We now show that both $\bpi{i}(\beta^i)$ and $\bri{i}(\beta^i))$, run on
  $\bv_i$, are incentive compatible and individually rational. First,
  buyer $i$ always prefers to win item $\k$ if she wins it according
  to this mechanism, since
  $v_i(\k) \geq \bv_i(\k) \geq \bp(\beta^i)_{\k}$. Thus, the item
  pricing mechanism is IR. Furthermore, an additive buyer $i$ has no
  reason to misreport $\v_i$; decreasing $\v_i(\k)$ does not affect
  the price of $\k$ but might cause her to lose $\k$ when she
  previously won (which, as before, she weakly prefers to win); nor
  will she want to increase $\v_i(\k)$, as it won't change
  $\bpi{i}(\beta^i)_{\k}$ but might cause $\bv_i(\k)$ to increase and
  allow her to win when she didn't previously, but only when
  $\bv_i(\k) < v_i(\k) \leq \max_{i'\neq i}v_{i'}(\k)$, so her price
  for $\k$ will be at least as large as $v_i(\k)$. Thus, running
  $\bpi{i}(\beta^i)$ on $\bv_i$ is also incentive-compatible for $v_i$.
  An analogous argument can be made for $\bri{i}(\beta^i)$ to prove its
  individual rationality and incentive compatibility.
\end{prevproof}


\begin{prevproof}{Lemma}{lem:independent}
  By assumption
  $((v_1(1), \ldots, v_n(1)), \ldots, (v_1(k), \ldots, v_n(k)))
  \sim \F^1\times \ldots \times \F^k$.
  Thus, for any function $f : \R^n \to \R^n$,
  \[(f(v_1(1), \ldots, v_n(1)) , \ldots, f(v_1(k), \ldots,
  v_n(k)))\sim \F'^1\times \ldots \times \F'^k,\]
  since $f$ is applied separately on each random variable drawn
  independently from a product distribution. Then, taking
  $f(v_1(\k), \ldots v_n(\k))_i = \bv_i(\k) = \v_i(\k)\cdot
  \mathbb{I}\lbrack[v_i(\k) > \max_{i'\neq i}v_{i'}(\k)\rbrack$
  proves the claim.
\end{prevproof}

\begin{prevproof}{Lemma}{lem:item-increase}
  First, notice that for any $\k$, $\bv_i(\k) > 0$ only if
  $v_i(\k) > \beta^i_k$.This implies that
  $\bv_i(\k) \geq \pik{i}{\k} > 0$ only if $v_i(\k) >
  \beta^i_\k$.
  Thus, if $\bv_i$ buys $\k$ at $\pik{i}{\k}$, she will also buy $\k$ at
  $\max (\pik{i}{\k}, \beta^i_k)$.  Finally,
  $\bpi{i}(\beta^i)(\k) \geq \pik{i}{\k}$, so the revenue of selling $\k$ is
  only larger. Thus, $\k$ is sold to $\bv_i$ by $\bpi{i}(\beta^i)$
  whenever it is sold to $\bv_i$ by $\np_{i}$, and is sold for a weakly
  larger payment, and the claim follows.
\end{prevproof}


\begin{prevproof}{Lemma}{lem:bundle-increase}
  For the set of items $\k$ such that $\bv_i(\k) > 0$, we know that
  $v_i(\k) > \beta^i_\k$. Thus, in particular,
  $\sum_{\k : \bv_i(\k) > 0} \bv_i(\k) = \sum_{\k : \bv_i(\k) > 0}
  v_i(\k) > \sum_{\k : \bv_i(\k) > 0} \beta^i_{\k}.$
  Thus, if $\sum_{\k : \bv_i(\k) > 0} \bv_i(\k) \geq \nri{i}$, it is
  also the case that
  $\sum_{\k : \bv_i(\k) > 0} \bv_i(\k) \geq \max(\nr_i, \sum_{\k :
    \bv_i(\k) > 0} \beta^i_{\k})$,
  so the bundle is sold to $\bv_i$ by $\bri{i}(\beta^i)$ whenever it
  was sold to $\bv_i$ by $\nri{i}$. As in the item pricing case, the
  revenue when the bundle is sold is weakly larger, so the claim
  follows.
\end{prevproof}


